A Broadband Conversion Loss Measurement Technique for Terahertz Harmonic Mixers

This letter presents an experimental characterization technique for assessing the performance of terahertz harmonic mixers across a wide frequency range. The total signal transfer loss of three mixers was measured in both up- and down-conversion configurations, and the conversion loss was determined through the solution of a linear system of equations. The proposed method uses LO signals with a frequency offset to ensure single sideband measurements, thereby eliminating the need for image-reject filters. The three-mixer method was verified by measurements of millimeter-wave mixers, which matched the traditional characterization method using a calibrated source and power meter. Given this successful millimeter-wave demonstration, we characterized three WM-86 Schottky diode x4-harmonic mixers from 2.2 to 3 THz. This technique presents a notable advantage for conducting broadband mixer characterizations, particularly in the terahertz frequency regime which lacks tunable, wide-band sources.

==> Chapter/Biography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{Photo/Divya.jpg}}]%
{Divya Jayasankar}
(S’19) received her B.E. degree in electronics and communication engineering in 2015 and the M.Sc. degree in wireless, photonics and space engineering from the Chalmers University of Technology, Gothenburg, Sweden, in 2019.
She is currently employed as an institute doctoral student at the Research Institutes of Sweden and Chalmers University of Technology. Her research interests include the development of THz mixers for future space applications and THz metrology. 

D. Jayasankar received the European Microwave Association (EuMA) internship award in 2021, the IEEE-MTTs graduate fellowship and the Roger Pollard fellowship for microwave measurements by ARFTG in 2022. She won second place in the best student paper competition in ISSTT conference held in Baeza, Spain in 2022. 
\end{IEEEbiography}


\begin{IEEEbiography}
{Theodore Reck} received his B.S. degree in electrical engineering from the University of Texas at Austin, Austin, TX, USA, in 2000, and his Ph.D. degree in electrical engineering from the University of Virginia, Charlottesville, VA, USA, in 2010.,From 2010 to 2013, he was a NASA Postdoctoral Fellow with the Jet Propulsion Laboratory (JPL) designing terahertz devices that utilize silicon micromachined packaging. From 2013 to 2018, he was a member of the Technical Staff with JPL developing terahertz components and systems. In 2018, he joined Virginia Diodes, Inc., as a Senior Engineer. His research interests include Schottky-diode mixers and multipliers, radio frequency microelectromechanical systems, and terahertz metrology.
\end{IEEEbiography}



\begin{IEEEbiography}
{Steven Durant} received the B.S. and M.S. degree in electrical engineering from the University of Virginia in 2010. He then joined Virginia Diodes Inc. developing custom terahertz systems and VNA extenders. His research interests include Schottky mixer design, filter design and VNA metrology. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{Photo/Jan.jpeg}}]%
{Jan Stake}
(S’95–M’00–SM’06) was born in Uddevalla, Sweden, in 1971. He received the M.Sc. degree in electrical engineering and the Ph.D. degree in microwave electronics from the Chalmers University of Technology, Gothenburg, Sweden, in 1994 and 1999, respectively.

In 1997, he was a Research Assistant with the University of Virginia, Charlottesville, VA, USA. From 1999 to 2001, he was a Research Fellow with the Millimetre Wave Group at the Rutherford Appleton Laboratory, Didcot, UK. He then joined Saab Combitech Systems AB, Linköping, Sweden, as a Senior RF/microwave Engineer, until 2003. From 2000 to 2006, he held different academic positions with the Chalmers University of Technology and from 2003 to 2006, he was also the Head of the Nanofabrication Laboratory, Department of Microtechnology and Nanoscience (MC2). During 2007, he was a Visiting Professor with the Sub-millimetre Wave Advanced Technology (SWAT) Group at Caltech/JPL, Pasadena, CA, USA. In 2020, he was a Visiting Professor at TU Delft. He is currently a Professor and the Head of the Terahertz and Millimetre Wave Laboratory, Chalmers University of Technology. He is also the Co-founder of Wasa Millimeter Wave AB, Gothenburg, Sweden. His research interests include graphene electronics, high frequency semiconductor devices, THz electronics, sub-millimetre wave measurement techniques (THz metrology), and THz in biology and medicine.
\newline
Prof. Stake served as the Editor-in-Chief for the IEEE Transactions on Terahertz Science and Technology between 2016 and 2018 and Topical Editor between 2012 and 2015.
\end{IEEEbiography}



\begin{IEEEbiography}
{Jeffrey Hesler} received the B.S.E.E. degree from Virginia Tech, Blacksburg, VA, USA, in 1989, and the M.S.E.E. and Ph.D. degrees from the University of Virginia, Charlottesville, VA, USA, in 1991 and 1996, respectively.,He is the Chief Technology Officer of Virginia Diodes Inc., Charlottesville, VA, USA, and a Visiting Research Assistant Professor at the University of Virginia. His career is focused on the creation of new technologies that are making possible the full exploitation of the Terahertz (THz) frequency band for scientific, defense, and industrial applications. He has authored and coauthored more than 150 technical papers in refereed international conferences and journals, given talks at THz-focused workshops and conferences such as IMS and EuMW. THz systems based on his innovative designs are now used in hundreds of research laboratories throughout the world.,Dr. Hesler is a member of IEEE TC MTT-4 on THz Technology and Applications and serves as a reviewer for a variety of the IEEE and IEE journals.

\end{IEEEbiography}




